AdANNS: A Framework for Adaptive Semantic Search

Web-scale search systems learn an encoder to embed a given query which is then hooked into an approximate nearest neighbor search (ANNS) pipeline to retrieve similar data points. To accurately capture tail queries and data points, learned representations typically are rigid, high-dimensional vectors that are generally used as-is in the entire ANNS pipeline and can lead to computationally expensive retrieval. In this paper, we argue that instead of rigid representations, different stages of ANNS can leverage adaptive representations of varying capacities to achieve significantly better accuracy-compute trade-offs, i.e., stages of ANNS that can get away with more approximate computation should use a lower-capacity representation of the same data point. To this end, we introduce AdANNS, a novel ANNS design framework that explicitly leverages the flexibility of Matryoshka Representations. We demonstrate state-of-the-art accuracy-compute trade-offs using novel AdANNS-based key ANNS building blocks like search data structures (AdANNS-IVF) and quantization (AdANNS-OPQ). For example on ImageNet retrieval, AdANNS-IVF is up to 1.5% more accurate than the rigid representations-based IVF at the same compute budget; and matches accuracy while being up to 90x faster in wall-clock time. For Natural Questions, 32-byte AdANNS-OPQ matches the accuracy of the 64-byte OPQ baseline constructed using rigid representations -- same accuracy at half the cost! We further show that the gains from AdANNS translate to modern-day composite ANNS indices that combine search structures and quantization. Finally, we demonstrate that AdANNS can enable inference-time adaptivity for compute-aware search on ANNS indices built non-adaptively on matryoshka representations. Code is open-sourced at https://github.com/RAIVNLab/AdANNS.

==> TabsNFigs/AdANNS_vs_AdaptiveInference.tex <==
\begin{figure}[b!]
\centering
\resizebox{\columnwidth}{!}{%
  \includegraphics[width=0.9\columnwidth]{TabsNFigs/sns_images/AdANNS_vs_Adaptive_Inference.pdf}
  }\vspace{-3mm}
    \caption{Compute-accuracy trade-off for the two variants of \AdANNS, \AdANNS-C \& \AdANNS-D on IVF. \AdANNS-C is better than \AdANNS-D due to the control during construction.}
  \label{fig:adannsd-compute}
  % \vspace{-3mm}
\end{figure}

==> TabsNFigs/Adaptive_Inference.tex <==
\begin{figure}[t!]
\centering
\resizebox{0.8\columnwidth}{!}{%
    % \vspace{5mm}
  \includegraphics[width=\columnwidth]{TabsNFigs/sns_images/Adaptive_Inference_vs_IVF_Top-1.pdf}
  }
    \caption{\AdANNS-IVF-D enables adaptive inference using low-dimensional \MRs on IVF built using 2048-d \MRs that can be used based on deployment requirements on a shared index/database.}
  \label{fig:adaptive-inference}
  % \vspace{-3mm}
\end{figure}

==> TabsNFigs/HNSW_1K-top1.tex <==
\begin{figure}[ht!]
\centering
  % \includegraphics[width=\columnwidth]{TabsNFigs/images/HNSW32 Top-1 vs Vector Dimensionality.pdf}
  % \includegraphics[width=\columnwidth]{TabsNFigs/sns_images/HNSW32 Top-1 vs Vector Dimensionality.pdf}
  \includegraphics[width=\columnwidth]{TabsNFigs/sns_images/IVF_top1_vs_compute.pdf}
  \vspace{-4mm}
    \caption{Variation of Top-1 Accuracy with increasing compute of MRL ResNet50 ImageNet-1K embeddings clustered with IVF-\MRL.}
    \vspace{-4mm}
  \label{fig:r50-ivf-1k-compute}
\end{figure}

==> TabsNFigs/HNSW_ivf_1K-r100.tex <==
% \begin{figure}[ht!]
% \centering
%   \includegraphics[width=0.47\columnwidth]{TabsNFigs/sns_images/HNSW32 Recall@100.pdf}
%     \includegraphics[width=0.47\columnwidth]{TabsNFigs/sns_images/IVF Recall@100.pdf}
%     \caption{Recall@100 of \MR compared to \RR baselines on ImageNet-1K with HNSW and IVF.}
%   \label{fig:r50-ivf-hnsw-1k-r100}
% \end{figure}

\begin{figure*}[t!]
\centering
\begin{subfigure}[]{.47\textwidth}
  \centering
  \includegraphics[width=\linewidth]{TabsNFigs/sns_images/IVF_Top-1_vs_Vector_Dimensionality.pdf}
  \caption{IVF top-1 accuracy}
  \label{fig:app-ivf-top1}
\end{subfigure}%
\begin{subfigure}[]{.47\textwidth}
  \centering
  \includegraphics[width=\linewidth]{TabsNFigs/sns_images/HNSW32_Top-1_vs_Vector_Dimensionality}
  \caption{HNSW top-1 accuracy}
  \label{fig:app-hnsw-top1}
\end{subfigure}
\begin{subfigure}[]{.47\textwidth}
  \centering
  \includegraphics[width=\linewidth]{TabsNFigs/sns_images/IVF_Recall_100.pdf}
  \caption{IVF Recall@100}
  \label{fig:app-ivf-r100}
\end{subfigure}%
\begin{subfigure}[]{.47\textwidth}
  \centering
  \includegraphics[width=\linewidth]{TabsNFigs/sns_images/HNSW32_Recall_100.pdf}
  \caption{HNSW Recall@100}
  \label{fig:app-hnsw-r100}
\end{subfigure}\\ \vspace{3mm}
\caption{Top-1 and Recall@100 of \MR compared to \RR baselines on ImageNet-1K with HNSW and IVF.}
\label{fig:r50-ivf-hnsw-1k-top1-r100}
\end{figure*}

==> TabsNFigs/MRL-HNSW.tex <==
% \begin{figure*}[ht!]
% \centering
% \begin{minipage}{.47\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{TabsNFigs/sns_images/IVF Top-1 vs Vector Dimensionality.pdf}
%   \caption{Comparison of ImageNet-1K Top-1 Accuracy variation with increasing ResNet50 embedding dimensionality $d$ of IVF-\MRL compared to IVF-\RR and Exact Search baselines.}
%   \label{fig:ivf-1k}
% \end{minipage}%
% \hspace{2mm}
% \begin{minipage}{.47\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{TabsNFigs/sns_images/HNSW32 Top-1 vs Vector Dimensionality.pdf}
%   \caption{Comparison of ImageNet-1K Top-1 Accuracy variation with increasing ResNet50 embedding dimensionality $d$ of HNSW-\MRL compared to HNSW-\RR and Exact Search baselines.}
%   \label{fig:hnsw-1k}
% \end{minipage}
% \end{figure*}

% \begin{figure}[t!]
% \centering
% \begin{subfigure}[]{.23\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{TabsNFigs/sns_images/IVF Top-1 vs Vector Dimensionality.pdf}
%   \caption{IVF}
%   \label{fig:ivf-1k}
% \end{subfigure}%
% \begin{subfigure}[]{.23\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{TabsNFigs/sns_images/HNSW32 Top-1 vs Vector Dimensionality.pdf}
%   \caption{HNSW32}
%   \label{fig:hnsw-1k}
% \end{subfigure}
% \vspace{-2mm}
% \caption{Comparison of ImageNet-1K 1-NN accuracy with increasing representation size $d$ using two popular indices -- (a) IVF and (b) HNSW. The gains in accuracy are extremely marginal at dimensionalities higher than 128-d -- thus making it an optimal choice for the accuracy-compute trade-off.}
% \label{fig:ivf-hnsw-1k}
% \end{figure}

\begin{figure}[b!]
\centering
\resizebox{0.8\columnwidth}{!}{%
\includegraphics[width=0.8\linewidth]{TabsNFigs/sns_images/HNSW32 Top-1 vs Vector Dimensionality.pdf}
}\vspace{-5mm}
\caption{Comparison of ImageNet-1K 1-NN accuracy with increasing representation size $d$ using HNSW. The gains in accuracy are extremely marginal at dimensionalities higher than 128-d -- thus making it an optimal choice for the accuracy-compute trade-off.}
\vspace{-5mm}
\label{fig:ivf-hnsw-1k}
\end{figure}

==> TabsNFigs/MRL-IVF_SearchProbes.tex <==
\begin{figure}[ht!]
\centering
  \includegraphics[width=\columnwidth]{TabsNFigs/images/MRL-IVF Top-1 vs. Search Probes.pdf}
    \caption{Top-1 Accuracy variation of MRL ResNet50 model on ImageNet-4K with increasing cluster search probes.}
  \label{fig:ivf-1k-searchprobes}
\end{figure}

==> TabsNFigs/MRL_PQ_Dims.tex <==
\begin{figure}[t!]
\centering
\resizebox{\columnwidth}{!}{%
  % \includegraphics[width=\columnwidth]{TabsNFigs/images/PQ Top-1 vs Vector Byte Size.pdf}
  \includegraphics[width=\columnwidth]{TabsNFigs/sns_images/PQ Top-1 vs Vector Byte Size.pdf}
  }
    \caption{The accuracy-compute trade-off across dimensionalities and 3 PQ compute budgets (16, 32 and 64 bytes). Each PQ budget has an optimal data dimensionality that is often not the highest/most informative owing to the hardness of clustering.}
  \label{fig:mrl-pq-dims}

\end{figure}

==> TabsNFigs/PQ_HNSWPQ_IVFPQ_Top1.tex <==
% \begin{figure*}[t!]
% \centering
% \begin{subfigure}[]{.47\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{TabsNFigs/sns_images/IVFPQ Top-1 vs Embedding Dimensionality.pdf}
%   \caption{IVFPQ}
%   \label{fig:ivfpq-top1}
% \end{subfigure}%
% \begin{subfigure}[]{.47\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{TabsNFigs/sns_images/HNSWPQ Top-1 vs Embedding Dimensionality.pdf}
%   \caption{HNSWPQ}
%   \label{fig:hnswpq-top1}
% \end{subfigure}
% \vspace{-2mm}
% \caption{Top-1 Accuracy of \MRL ResNet50 model compared to baselines on ImageNet-1K.}
% \label{fig:ivfpq-hnswpq}
% \end{figure*}

\begin{figure*}[t!]
\centering
\begin{subfigure}[]{.31\textwidth}
  \centering
  \includegraphics[width=\linewidth]{TabsNFigs/sns_images/PQ_Top-1_vs_Vector_Byte_Size.pdf}
  \caption{PQ}
  \label{fig:pq-top1}
\end{subfigure}
\begin{subfigure}[]{.32\textwidth}
  \centering
  \includegraphics[width=\linewidth]{TabsNFigs/sns_images/IVFPQ_Top-1_vs_Embedding_Dimensionality.pdf}
  \caption{IVFPQ}
  \label{fig:ivfpq-top1}
\end{subfigure}%
\begin{subfigure}[]{.31\textwidth}
  \centering
  \includegraphics[width=\linewidth]{TabsNFigs/sns_images/HNSWPQ_Top-1_vs_Embedding_Dimensionality.pdf}
  \caption{HNSWPQ}
  \label{fig:hnswpq-top1}
\end{subfigure}
\caption{Evaluation of accuracy-compute trade-off for (a) standard PQ, (b) IVFPQ and (c) HNSWPQ indices built on varying dimensional \MRs and \RRs. We investigate 16, 32, and 64-byte PQ budgets and find that the highest-dimensional representation need not be the most aligned for quantization owing to hardness of clustering.}
\label{fig:ivfpq-hnswpq}
\end{figure*}

==> TabsNFigs/Recall_Curves_1K.tex <==
% \begin{figure*}[t!]
% % \vspace{-3mm}
% \centering
% \resizebox{2\columnwidth}{!}{%
% % \includegraphics[width=0.8\columnwidth]{TabsNFigs/images/Screen Shot 2022-05-12 at 7.10.36 PM.png}
% % \hspace{-10mm}
% \begin{tabular}{ccc}
% \includegraphics[width=\columnwidth]{TabsNFigs/sns_images/R50+IN1K_ R1@1 for Clustering.pdf}
% % \includegraphics[width=\columnwidth]{TabsNFigs/images/R50+IN4K_ R1@1 for Clustering.pdf} 
% \includegraphics[width=\columnwidth]{TabsNFigs/sns_images/R50+IN1K_ R1@1 for HNSW.pdf}
% \end{tabular}
% % }\\
% }
% % \vspace{-3mm}
% % \vspace*{-5pt}
% \caption{k-Recall@N for ResNet50 MRL models on ImageNet-1K compared to baselines for ANNS with k-Means clustering and HNSW. General trends show a) an intuitive increase in recall with increasing search probes b) for fixed search probes, a decrease in recall with increasing search dimensionality $d$.} 
% % }
% % \vspace{-5mm}
% \label{fig:r50-recall-score}
% \end{figure*}

\begin{figure}[b!]
\centering
\begin{subfigure}[]{.23\textwidth}
  \centering
  \includegraphics[width=\linewidth]{TabsNFigs/sns_images/R50+IN1K_R1_1_for_Clustering.pdf}
  \caption{IVF}
  \label{fig:ivfpq-recall-score}
\end{subfigure}%
\begin{subfigure}[]{.23\textwidth}
  \centering
  \includegraphics[width=\linewidth]{TabsNFigs/sns_images/R50+IN1K_R1_1_for_HNSW.pdf}
  \caption{HNSW}
  \label{fig:hnswpq-recall-score}
\end{subfigure}
\vspace{-2mm}
\caption{Recall score plots with 1-Recall@1 for ImageNet-1K using IVF and HNSW on \MRs and \RRs of 64, 256 \& 2048-d.}
\label{fig:r50-recall-score}
\end{figure}

==> TabsNFigs/Recall_Curves_4K.tex <==
\begin{figure*}[ht!]
% \vspace{-3mm}
\centering
\resizebox{0.8\columnwidth}{!}{%
% \includegraphics[width=0.8\columnwidth]{TabsNFigs/images/Screen Shot 2022-05-12 at 7.10.36 PM.png}
% \hspace{-10mm}
\begin{tabular}{ccc}
\includegraphics[width=0.8\columnwidth]{TabsNFigs/sns_images/R50+IN4K_R40_2048_for_Clustering.pdf}
\includegraphics[width=0.8\columnwidth]{TabsNFigs/sns_images/R50+IN4K_R1_1_for_Clustering.pdf} 
% \includegraphics[width=\columnwidth]{TabsNFigs/images/R50+IN1K_ R40@2048 for Clustering.pdf}
% \includegraphics[width=\columnwidth]{TabsNFigs/images/R50+IN1K_ R40@2048 for HNSW.pdf}
\end{tabular}
% }\\
}
% \vspace{-3mm}
% \vspace*{-5pt}
\caption{k-Recall@N for IVF-\MR-$d$ on ImageNet-4K for $d\in\{8,64,256,2048\}$. Other embedding dimensionalities, HNSW-\MR and \RR baselines are omitted due to high compute cost. We observe that trends from ImageNet-1K with increasing $d$ and $n_p$ extend to ImageNet-4K, which is $4\times$ larger.} 
% }
% \vspace{-5mm}
\label{fig:app-rk@N-4K}
\end{figure*}

==> blocks.tex <==
\section{Further Analysis on ANNS Components}
\label{sec:blocks}

State-of-the-art ANNS pipelines~\citep{johnson2019billion,jayaram2019diskann} use two other key techniques alongside IVF: (a) Product Quantization (PQ) and (b) Hierarchical Navigable Small World graphs (HNSW). Naturally, a question arises if \AdANNS can be combined with such ANNS components. While we theoretically argue about the complementary nature of \AdANNS to PQ and HNSW (Section~\ref{sec:adanns}), here we provide preliminary results in that direction. We show that: (a) PQ-based approximate distance computation is complementary to \MRs and can be easily added to \AdANNS-D; (b) \MRs are better than \RRs when using HNSW and PQ can be leveraged on top of them to find optimal accuracy-compute trade-off. For simplicity of exposition, and highlighting the key aspects of \AdANNS, our primary adaptation and experiments are on IVF which is another state-of-the-art ANNS data structure. 


% \begin{itemize}
%     \item PQ -- MRl vs FF and low-d vs high-d
%     \item IVF -- MRL vs FF and compute \& recall score plots
%     \item HNSW -- MRL vs FF and low-d vs high-d \& recall score plots 
%     \item IVFPQ -- fixed clsuters, MRL vs FF on PQ
%     \item HNSWPQ -- fixed HNSW config, MRL vs FF on PQ
% \end{itemize}

% \begin{itemize}
%     \item Compressebility of Representations
%     \item Adaptive deployment for search -- LSHish stuff? 
% \end{itemize}



% In this section we evaluate the strength of flexible MRL representations for a) Clustering in low-dimensional subspaces b) Quantization for lowered memory cost b) Search space partitioning for approximate nearest neighbors search (ANNS). A bulk of our experimentation was carried out via Faiss~\cite{johnson2019billion}, a library for efficient similarity search and clustering.
% \paragraph{Datasets} MRL for flexible ANNS was evaluated on ImageNet-1K~\cite{deng2009imagenet}, ImageNet-V2~\cite{recht2019imagenet} and ImageNet-4K~\cite{kusupati22matryoshka}.
% \paragraph{Hardware} All ANNS experiments (HNSW, HNSWPQ, IVFPQ) were run on an Intel Xeon 2.20GHz CPU with 12 cores. Clustering (IVF, k-Means), Adaptive Retrieval (Adaptive  k-Means + Linear Scan) and Exact search experiments were run with CUDA 11.0 on a A100-SXM4 NVIDIA GPU with 40G RAM.

% Apart from powering adaptive ANNS, adaptive representations also find the data dimensionalities for near-optimal accuracy-compute trade-offs. A typical ANNS pipeline consists of many such building blocks which are often complementary. Finding the optimal data dimensionality of the learned representation at each stage will significantly improve the search Pareto frontier. We search for optimal data dimensionalities for product quantization (PQ), data structures like IVF and HNSW, and composite indices of IVF+PQ and HNSW+PQ. 


\subsection{Product Quantization}
\label{subsec:pq}
% \input{TabsNFigs/MRL_PQ_Dims.tex}
% \input{TabsNFigs/PQ_HNSWPQ_IVFPQ_Top1.tex}
Product quantization (PQ)~\citep{jegou2010product} works by splitting a $d$-dimensional real vector into $m$ sub-vectors and quantizing each sub-vector with an independent $2^b$ length codebook across the database. After PQ each $d$-dimensional vector can be represented by a compact $m\times b$ bit vector -- we fix $b=8$ making the vectors $m$ bytes long. The generality of PQ encompasses scalar/vector quantization~\citep{gray1984vector,lloyd1982least} as special cases. While, significant work has been done to improve PQ further~\citep {ge2013optimized,chen2020differentiable}, we only experiment with standard PQ as the improvements are complementary (See Appendix~\ref{app:quantization}).

Figure~\ref{fig:pq-top1} shows that often lower-dimensional representations provide better compute-vs-accuracy trade-off for PQ.  For 32-byte PQ, a deployment default, it is better to use a 128-d representation instead of the full 2048-d. At the same time, we also find that \MRs are more aligned for PQ owing to the information packing compared to \RRs. For a fixed budget of PQ, the accuracy steadily increases till a specific dimensionality and then deteriorates. Finally, we also note that on ImageNet-1K, a net 2-bit quantization seems to work the best (ie., 32-d is the best for 8-byte PQ). See Appendix~\ref{app:quantization} for evaluation across more PQ budgets that further strengthen the observations. This shows that PQ is complementary to low-dimensional \MRs and can be combined with \AdANNS-D to further speed-up inference.


% All these results transfer to the cases that use PQ as part of composite indices (Section~\ref{subsec:composite-indices}) for faster distance computation ie., for an IVF + 32-byte PQ; IVF can be built on 2048-d, while the best 32-byte PQ can be obtained using 128-d.

% \todo{Key Observation: Low-d representation are better compute budgets used in the deployment and MRL is much better than FF.}

% \todo{Edit} Vector Quantization was explored through Product Quantization (PQ) and its optimized variant OPQ~\cite{ge2013optimized}. Note that scalar quantization is a special case of PQ when we use $d$ sub-quantizers across the entire vector, i.e. $m = d$. As shown in Fig.~\ref{fig:teaser-pq}, MRL provides more than 1\% Top-1 increase over baselines for compression of $32$ bytes or less. It is also notable that the highest Top-1 for a fixed PQ compression $m$ is not from the highest dimensionality $d$. This indicates the importance and potential of flexible representations for the optimal $(m, d)$ PQ compression.

% \todo{Experiments for PQ with varying dims for MRL and FF + Figure}

% \subsection{Inverted File Index}
% \label{subsec:ivf}


% Figure~\ref{fig:ivf-1k} shows that for a fixed inverted file index (IVF) configuration, with 1024 clusters and 1 probe, the accuracy starts to saturate at much lower dimensions (around 64-d) than the highest dimension (2048-d). As the compute overhead of IVF scales linearly with dimensionality, low-dimensional representations will result in optimal accuracy-compute trade-off. We also note that \MRs are consistently better than \RRs across all accuracy-compute constraints strengthening the choice of matryoshka representations for ANNS. However, the compute footprint in IVF also depends on the number of clusters as it dictates the number of data points per cluster. Please refer to Appendix~\ref{app:clustering} for the exhaustive evaluation of IVF across more accuracy-compute choices as well as specific implementation details. 

% However, the compute footprint in IVF also depends on the number of clusters as it dictates the number of data points per cluster. We did an exhaustive design space search across dimensionality, number of clusters, and probes as each aspect affects different overheads in large-scale systems. For example, reducing the  clusters increases the speed of the initial cluster assignment (cached load-balancer) while also increasing the linear search overhead within each cluster. So for each such configuration, there exists a data dimensionality that does justice to the accuracy-compute trade-off. 

% Figure~\ref{fig:ivf-1k} shows the accuracy-compute trade-off of selected configurations for IVF. It is evident that with a fine-grained search of IVF design space, we can obtain the same accuracy as a high-dimensional configuration with significantly lower (up to $10\times$) compute. We also note that \MRs are consistently better than \RRs across all accuracy-compute constraints strengthening the choice of matryoshka representations for ANNS. Please refer to Appendix~\ref{app:clustering} for the exhaustive evaluation of IVF across more accuracy-compute choices as well as specific implementation details. 

% \todo{Key Takeaway: Accurate lower-d representations are better for IVF. Fine-grained design space search helps with improving pareto-optimality}.

% \subsection{HNSW}
% \label{subsec:hnsw}
% Hierarchical Navigable Small World graph (HNSW) is a state-of-the-art ANNS index with more memory overhead compared to IVF. HNSW is often the go-to out-of-the-box choice for high-accuracy ANNS~\citep{Github:clip_retrieval}. We investigate the compute-accuracy trade-off of the default HNSW index~\citep{johnson2019billion} built on varying capacity \MRs and \RRs. We find that HNSW is slightly more accurate than IVF but comes with a large index memory overhead. Figure~\ref{fig:r50-ivf-hnsw-1k-top1-r100} in Appendix~\ref{app:ANNS} shows that the accuracy gain is marginal after certain data dimensionality for HNSW, but the compute and memory cost grow linearly with $d$ -- making low-dimensional representation better for the accuracy-compute trade-off. For example, the accuracy gain from 128-d to 2048-d \MR is marginal while the overhead increases $16\times$. Similar to the observations in PQ and IVF, \MRs outperform \RRs even for graph-based while showing that \MRs are complementary to HNSW as well.

% \todo{Key Takeway: Better low-d representations exists for HNSW as well.}

% \input{TabsNFigs/HNSW_1K-top1.tex}



\subsection{Composite Indices -- IVFPQ \& HNSWPQ}
\label{subsec:composite-indices}
Composite indices represent the existing adaptivity in ANNS pipelines. An ANNS data structure is often built on a high-dimensional \RR, but can not afford distance computation with the same. In these cases, we use cheaper distance computation through dimensionality reduction -- typically through PQ~\citep{jayaram2019diskann}. Composite indices trade off the accurate construction of the expensive structure with efficient inference. 

Figures~\ref{fig:ivfpq-top1} and \ref{fig:hnswpq-top1} show that even for composite indices (IVFPQ and HNSWPQ), lower dimensions result in a better accuracy-compute trade-off as they can cluster and quantize better compared to higher-dimensions. The trends of IVFPQ and HNSWPQ follow that of PQ where \MRs are consistently better than \RRs and the best accuracy peaks at a much lower dimension than 2048-d.


A key thing to note is that the \AdANNS-D proposed for adaptive inference in Section~\ref{sec:adanns-ivf-d} is a generalized variant of composite indices where data structure construction and inference happen with representations of different capacities. While \AdANNS-D uses low-d \MRs for distance computation, as observed here they also can result in better PQ vectors for further speed-ups. The design space of composite indices blows up when using adaptive representations hence using \MRs for ANNS design and deployment can result in a smooth and flexible inference time adoption with minimal design search overhead.




